Experimental quantum memristor

Quantum computer technology harnesses the features of quantum physics for revolutionizing information processing and computing. As such, quantum computers use physical quantum gates that process information unitarily, even though the final computing steps might be measurement-based or non-unitary. The applications of quantum computers cover diverse areas, reaching from well-known quantum algorithms to quantum machine learning and quantum neural networks. The last of these is of particular interest by belonging to the promising field of artificial intelligence. However, quantum neural networks are technologically challenging as the underlying computation requires non-unitary operations for mimicking the behavior of neurons. A landmark development for classical neural networks was the realization of memory-resistors, or "memristors". These are passive circuit elements that keep a memory of their past states in the form of a resistive hysteresis and thus provide access to nonlinear gate operations. The quest for realising a quantum memristor led to a few proposals, all of which face limited technological practicality. Here we introduce and experimentally demonstrate a novel quantum-optical memristor that is based on integrated photonics and acts on single photons. We characterize its memristive behavior and underline the practical potential of our device by numerically simulating instances of quantum reservoir computing, where we predict an advantage in the use of our quantum memristor over classical architectures. Given recent progress in the realization of photonic circuits for neural networks applications, our device could become a building block of immediate and near-term quantum neuromorphic architectures.

==> SECTIONS/numerical_revised.tex <==
Using measurements to introduce nonlinearities is a well-known paradigm in quantum photonic computing \cite{Knill2001,Raussendorf2001}. However, two fundamental differences set our photonic memristor apart from previous proposals. First, we implement a nonlinearity at a single-photon level without using trial and errors, ancillary photons, or other experimental overheads, which constitute the strongest limitation to schemes such as KLM \cite{Knill2001} or MBQC \cite{Walther2005}. This is possible because we accept a partial decoherence of the final output quantum state. Second and most importantly, we introduce a memory effect, which enables quantum optical networks to produce a time-correlated output, a feature which, to the best of our knowledge, was never explored before.

\begin{figure*}
    \centering
    {\includegraphics[width=.9\textwidth]{Figures/Digit_reservoir.png}}
    \caption{\textbf{Quantum memristor based reservoir computer.}(a)A fixed linear optical network is connected to a quantum memristor array. After propagating through this optical network, photon counters on each mode record the correlated output configurations which serve as the output data of the reservoir.
    (b)An unknown input quantum state $\ket{\phi_{in}}$ is fed into the quantum reservoir which acts on it in a nontrivial manner. The output statistics are then fed to a small neural network. This is then trained on these fixed outputs via backward propagation. (c)Digital images are encoded into a quantum state before being fed into the optical reservoir which produces a final state that is correlated with the image content. Image classification using the same network topology as in (b) may then be performed by training on a number of such reservoir output examples.}
    \label{fig::topology}
\end{figure*}

Consider a typical linear optical network such as the one schematised in Fig.\! \ref{fig::topology}(a). Quantum optical processing can be approximated as the action of linear operators on a Hilbert space whose dimension grows as ${m+p-1 \choose p}$ in the number of optical modes $m$ and $p$ photons present. This means that enormous amounts of information may be manipulated with relatively small spatial footprint and physical resources. Coupling this structure with nonlinear, stateful devices such as memristors that extend such manipulation through time as correlated operators, the state space becomes effectively infinite, limited only by our ability to control it.

It is in such architectures that the concept of reservoir computing comes to the fore\! \cite{Nakajima2017, tanaka2019, Nakajima2019}. In this computational model a large, randomly configured, and generally nonlinear physical system is exploited to perform computationally expensive operations on input information for free. The output of the reservoir can be configured to have a much smaller dimension than that of the input space. The task then becomes to interpret such output, which is assumed to be computationally less demanding than directly processing the input data itself. In Fig.\! \ref{fig::topology}(a) we introduce our model of such a quantum-photonic reservoir computer. The reservoir channel consists of an optical array constructed by fixed beam splitters (similarly to a recently proposed scheme\! \cite{Paterek2019}) that distributes coherent quantum information encoded in three photons across nine modes, before being fed to an array of quantum memristors that finally leads to a collection of photon counters on each mode. The array of photon counters forms the input to a small software-defined neural network which is then trained to interpret such data. 

One of the unique features of our architecture is that it can be applied to tasks that reside both in the classical and the quantum domains. A well-known, traditionally hard quantum task is, for instance, entanglement detection where one wishes to identify if an unknown quantum state contains any entanglement. This is typically performed by measuring observables called entanglement witnesses and using them to estimate the likelihood of the state containing some measure of entanglement\! \cite{Eisert2007}. Here we instead feed the unknown state directly to the reservoir (see Fig.\! \ref{fig::topology}(b)), where the presence of the memristors allows for a much more sophisticated map than a simple observable, and train the neural network to interpret the output. A small, fully connected, three-layer network of just two thousand parameters trained on one thousand examples, is able to identify entanglement with 89\% accuracy on one thousand, never-before-seen, 144-dimensional states. Though such results are hardly competitive with respect to dedicated, state-of-the-art techniques\! \cite{Saggio2019}, it is nevertheless impressive that such a general and broadly defined architecture performs well on a purely quantum information based task.

In a similar vein, a paradigmatic learning task in the classical domain is the classification of images of hand-written digits (see Fig.\! \ref{fig::topology}(c)). We consider a subset of images from the MNIST\! \cite{lecun2010mnist, tensorflow2015-whitepaper} database with digits zero, three and eight, and chosen for their vertical similarity. Each image is a matrix of 22 x 20 pixels after removal of borders, which are converted to binary values via thresholding function. The columns of these images then form binary strings of 22 bits and each string is encoded on the corresponding ordered eigenvector of the photonic Hilbert space and fed into the reservoir. After the last string has been sent through, the resulting vector of photon counters is interpreted by the neural network. Note that, because of the memristors, this final vector is correlated with all the previous iterations, i.e. with the whole image. With a fully connected three-layer neural network consisting of just three thousand tunable parameters we train on a small set of one thousand images over five epochs. This achieves a classification accuracy of 93\% on one thousand never-before-seen samples. 

This final result shows that a small quantum-optical reservoir equipped with quantum memristors and limited machine learning leads to exceptional performance compared to classical networks, requiring both less computational power to train the network and far fewer training examples. This latter point is especially advantageous given that the primary contributor to scalability problems for machine learning is both the amount of training data required to achieve worthwhile performance and the associated computational cost in using it. Importantly, the encoding we have chosen also has the side benefit of mapping groups of similar binary strings to similar regions of Hilbert space. This results in a high degree of robustness against noise in the quantum reservoir, as small fluctuations in the input state and action of the reservoir will yield similar expectation values in the memristors, and so similar feature vectors for the neural network to interpret. Quantum reservoir processing thus offers an immediately viable alternative for quantum enabled machine learning that can operate on both classical and quantum data with no architectural changes.


==> SECTIONS/numerical_revised_revised.tex <==
Neural networks are known to be very effective in computational tasks where a small amount of information needs to be extracted from a very large amount of data. One of these tasks, often used as a benchmark, is the recognition of images of handwritten digits \cite{lecun2010mnist}. A simple neural approach to this problem is schematised in Fig. \ref{fig_newnet}a. One can feed each pixel of the image to a neuron in the first layer of the network, and "train" the network to identify the digit by switching on the correct neuron of the last layer. Such techniques can identify handwritten digits with an accuracy of above 90\%, reaching more than 99\% in the most sophisticated approaches \cite{Weber2013}, but they typically require the active tuning of a large number of parameters. As a result, the amount of data and the computational cost required for training represent the main limiting scaling factor for these architectures.

The core idea of reservoir computing \cite{Herbert2001, Maass2002} is that the first layers of the network, which deal with the bulk of the input data and are therefore the most computationally expensive, do not necessarily need to be actively controlled. Instead, one can substitute them with a large, randomly configured, uncontrolled physical system — a reservoir — whose output dimension is assumed to be much smaller than that of the input data itself (see Fig. \ref{fig_newnet}b).  Training the rest of the network to interpret the  output  of  the  reservoir  turns  out  to  be  a  much  simpler computational tasks. In fact, it was shown that the exploitation of reservoirs leads to outstanding performance requiring lower training costs compared to conventional strategies  \cite{tanaka2019}.

Any physical system that is large enough to meaningfully encode the input data can be used as a reservoir. Reservoirs based on classical memristors have been already demonstrated experimentally \cite{Du2017,Moon2019}, and a few examples of quantum reservoirs have been proposed \cite{Nakajima2017,Paterek2019, Nakajima2019}. Here we propose and numerically evaluate a quantum photonic reservoir computer, where the reservoir is constructed as a quantum optical network equipped with quantum memristors as schematised in Fig. \ref{fig_newnet}c. A fixed matrix of beam-splitters distributes coherent information encoded on three photons across nine optical modes (not dissimilarly to other recent proposals \cite{Nakajima2019,Paterek2019}). These are then fed to the input ports of three memristors. An array of photon counters record the overall output of the reservoir, which is fed to a small software-defined neural network. 
Such a system, which is within the reach of current integrated photonic technology, immediately yields three striking advantages. First, when using an integrated photonic processor where $p$ photons are processed through $m$ optical modes, then a large state space becomes available that grows as ${m+p-1 \choose p}$. This means that enormous amounts of information may be manipulated with relatively small spatial footprint and physical resources. Second, the quantum memristors introduce a classical memory effect, which enables a quantum photonics network to produce a time-correlated output, a feature which, to the best of our knowledge, has never been explored before. Third, integrating classical data processing and classical feedback within a quantum system means that the architecture is applicable to both classical and quantum learning tasks.

As an example of classical task, we consider images of handwritten digits "0", "3" and "8" from the MNIST database \cite{lecun2010mnist}. 
Each image is cropped to $22\times20$ pixels converted to binary values via a threshold function. The columns then form binary strings of 22 bits, which are encoded in the corresponding ordered eigenvector of the photonic state space and fed to the reservoir one at a time (see Fig. \ref{fig_newnet}c). The output of the last column, which is correlated with all the previous columns because of the memory effect in the quantum memristors, is interpreted by the neural network. Simulations of a three-layer network consisting of under 2000 tunable parameters and trained by 1000 images over ten epochs achieved an identification accuracy of 98\% on never-before seen test images. This state-of-the-art accuracy is remarkable for such small-scale physical system 
and training resources. Furthermore, the specific type of encoding we have chosen has
shown high resilience against significant simulated noise in the input state and in the action of the reservoir.

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{Figures/neural_network.pdf}
    \caption{\textbf{Quantum reservoir computing.} \textbf{(a)} A classical neural approach to image classification. Each pixels of the image is fed to the first layer of the network, which is connected to a number of hidden layers leading to the final layer. The network can be trained to correctly identify the handwritten digit by switching on the corresponding neuron of the last layer. \textbf{(b)} Reservoir computing: the first layers of the network are substituted by a fixed, uncontrolled physical system (reservoir). The rest of the network is trained to interpret the output of the reservoir, leading to higher computational efficiency. \textbf{(c)} A quantum reservoir computer based on quantum memristors. The reservoir consists of an array of fixed beam splitter distributing coherent quantum information across nine optical modes, which are then fed to the input of three memristor. The columns of the image are encoded and sent to the reservoir one at a time. The memristors extend the correlations of the output across the entire time sequence, so that the output of the last column is correlated with the whole image. The rest of the network is trained to interpret such output. \textbf{(d)} The same architecture is used to perform entanglement detection. The quantum neural network can be trained to detect whether an unknown input state is entangled or not.}
    \label{fig_newnet}
\end{figure*}

On the other hand, a paradigmatic task in the quantum domain is entanglement detection, where one wishes to identify whether an unknown quantum state is entangled or not. Here we feed such unknown quantum states to the reservoir (see Fig. \ref{fig_newnet}d) and train the neural network to interpret the output.  According to our numerical simulations, a small, fully connected, three-layer network of just 200 parameters trained on 2000 examples, is able to identify entanglement with 85\% accuracy on 100-dimensional states. Though such results are hardly competitive with respect to dedicated, state-of-the-art techniques  \cite{Saggio2019}, it is nevertheless impressive that such a general and broadly defined architecture, equipped with an extremely small neural network, performs well also on purely quantum information tasks.

